Perturbing AGN Accretion Disks with Stars and Moderately Massive Black Holes: Implications for Changing-Look AGN and Quasi-Periodic Eruptions

We present a model that explains some extreme variability phenomena observed in active galactic nuclei (AGN). In this model, an orbiting companion interacts with the accretion disk surrounding the central supermassive black hole (SMBH). This interaction excites spiral density waves, leading to bursts of mass inflow lasting a few orbital timescales, whose mass content depends sensitively on the sphere of influence of the orbiting companion. To explain changing-look (CL) AGN, we find that lighter SMBH companions are necessary, while we generally exclude stellar companions. The moderately massive black hole perturber must be on a highly eccentric orbit in order to account for the non-repeating nature of most CL AGN. When applied to quasi-periodic eruptions (QPEs), we find that stars with highly eccentric orbits and close pericenter passages can produce accretion flares with QPE-like characteristics. For many QPEs, low-mass main-sequence stars or stripped-envelope stars are required. Although moderately massive black hole perturbers could also match the observed properties of QPEs, the gravitational-wave merger timescales of such binary systems are prohibitively short.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{braket}
%\usepackage{amsmath}
\usepackage[utf8]{inputenc}
\usepackage [greek,british]{babel}
\usepackage [autostyle, english = american]{csquotes}
\MakeOuterQuote{"}
\newenvironment{rcases}
  {\left.\begin{aligned}}
  {\end{aligned}\right\rbrace}
  
  \usepackage[OT2,T1]{fontenc}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{floatflt}
%\usepackage[explicit]{titlesec}
\usepackage{wrapfig}
\usepackage[table,xcdraw,svgnames]{xcolor}
\usepackage{tabu}
\usepackage{appendix}
\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\usepackage[colorlinks]{hyperref} %

\newcommand{\pder}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\no{\noindent}
% Ecrire sa thèse en Français
% http://www.theses.ulaval.ca/wiki/index.php?title=Latex:R%C3%A9daction_en_fran%C3%A7ais

%\usepackage[T2A,T1]{fontenc}
%\usepackage{newpxtext,newpxmath}
\usepackage{newtxtext,newtxmath}
\usepackage{icomma}
\usepackage{microtype}
\usepackage[font=small,labelfont=bf]{caption}

%\usepackage{ae}
%\usepackage{aeguill}
%\usepackage{fancyhdr}
%\usepackage{subfig}
\usepackage{pdfpages}
\usepackage{url}
\usepackage{verbatim}
\usepackage{comment}
\usepackage{ulem}
\usepackage{color}
\usepackage{xspace}
%\usepackage{hyperref}
\usepackage{floatrow}
\usepackage{geometry}
\usepackage{rotating}
\usepackage{wallpaper}
  \usepackage{eso-pic}
\setlength{\headheight}{15pt} 
% Mise en page
\usepackage[rightcaption]{sidecap}
%\newcommand{\noMinitocPlease}{true}
%\usepackage{fancyhdr}
\ifx\noMinitocPlease\undefined
\usepackage{minitoc}
\mtcselectlanguage{british}
\else
\usepackage{mtcoff}
\fi

%\DeclareUnicodeCharacter{00A0}{ }

\setcounter{tocdepth}{3}
\setcounter{secnumdepth}{3}

%\usepackage{braket}

\usepackage{a4wide} 
%\usepackage{vmargin}
%\setmarginsrb{2cm}{1cm}{2cm}{1cm}{1cm}{1cm}{1cm}{1cm}
%\def\clearpage{\hspace{1cm}}
\usepackage{version}

%\usepackage[final]{pdfpages}
% \includepdf[pages=1-20]{fichier.pdf}

%% entete Audrey
%\usepackage[cyr]{aeguill}
%\usepackage{float} 
\usepackage{caption}

%----------------------------------------------------------------------------
%macro pour activer ou desactiver l'incrementation de la table des matières
%---------------------------------------------------
\makeatletter
\let\original@addcontentsline\addcontentsline
\newcommand{\dummy@addcontentsline}[3]{}
\newcommand{\DeactivateToc}{\let\addcontentsline\dummy@addcontentsline}
\newcommand{\ActivateToc}{\let\addcontentsline\original@addcontentsline}
\makeatother


%----------------------------------------------------------------------------
%mise en page
%----------------------------------------------------------------------------
\usepackage{fancyhdr}
\pagestyle{fancy}

%----------------------------------------------------------------------------
%en tête du haut
%----------------------------------------------------------------------------
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\chaptermark}[1]{\markboth{\chaptername~\thechapter{} : #1}{}}
\renewcommand{\sectionmark}[1]{\markright{\thesection{} \ #1}}
\renewcommand{\sectionmark}[1]{\markright{\thesubsection{} \ #1}}
\lhead[]{\textsl{\rightmark}}
\rhead[\textsl{\leftmark}]{}

%----------------------------------------------------------------------------
%en tête du bas
%----------------------------------------------------------------------------
%\renewcommand{\footrulewidth}{1pt}
\fancyfoot[C]{\thepage} 

%----------------------------------------------------------------------------
% dédicace
%----------------------------------------------------------------------------
%\usepackage{multicol}
%\usepackage[linktocpage]{hyperref}
\usepackage{epigraph}
\newcommand{\dedicace}[1]{{%
\clearpage
\pagestyle{empty}
\setlength{\beforeepigraphskip}{10\baselineskip}
\setlength{\epigraphrule}{0pt}
%\epigraphtextposition{flushright}
\mbox{}
\epigraph{\itshape #1}{}}}

%----------------------------------------------------------------------------
% épigraphe
%----------------------------------------------------------------------------
\newcommand{\epigraphe}[2]{{%
\clearpage
\pagestyle{empty}
\setlength{\beforeepigraphskip}{10\baselineskip}
\mbox{}\epigraph{#1}{#2}}}

\newpage
\makeindex
%\renewcommand{\sc}{\textsc}
%\renewcommand{\bf}{\textbf}
%\renewcommand{\comment}[1]{({\textit *** #1 ***})}
\newcommand{\mathnotation}[2]{\newcommand{#1}{\ensuremath{#2}\xspace}}
\newcommand{\caca}[1]{\sout{#1}}
\renewcommand{\caca}[1]{}
\newcommand{\todo}[1]{\textcolor{red}{#1}}
%\renewcommand{\todo}[1]{#1}
\newcommand{\com}[1]{\textcolor{red}{(!!! #1 !!!)}}
\renewcommand{\com}[1]{}
\newcommand{\bof}[1]{\uwave{#1}}
\renewcommand{\bof}[1]{#1}
\newcommand{\xja}[1]{\uwave{#1}}
\renewcommand{\xja}[1]{#1}

\renewcommand{\epsilon}{\varepsilon}

%% Math notations ------------------------

\mathnotation{\mt}{m_t^* \xspace}
\mathnotation{\ml}{m_l^* \xspace}

\mathnotation{\VGone}{V_{g1}}
\mathnotation{\VGtwo}{V_{g2}}
\mathnotation{\Vback}{V_{bg}}
\mathnotation{\MUs}{\mu_{F,s}}
\mathnotation{\MUd}{\mu_{F,d}}

\mathnotation{\VGi}{{V_\mathrm{g \mathit{i}}}}
\mathnotation{\DVGi}{V_{\mathrm{g} \mathit{i}}^{\mathrm{AC}}}
\mathnotation{\DVGone}{V_{\mathrm{g} 1}^{\mathrm{AC}}}
\mathnotation{\DVGtwo}{V_{\mathrm{g} 2}^{\mathrm{AC}}}
\mathnotation{\VGonedc}{{V_{\mathrm{g1}}^{\mathrm{DC}}}}
\mathnotation{\VGtwodc}{{V_{\mathrm{g2}}^{\mathrm{DC}}}}
\newcommand{\VGidc}{$V_{\mathrm{g \mathit{i}}}^{\mathrm{DC}}$}
\newcommand{\Gin}{\Gamma_{\mathrm{in}}}
\newcommand{\vg[1]}{$V_{\mathrm{g#1}}$}
\newcommand{\diff[2]}{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\mathnotation{\ECM}{U'}
\newcommand{\DPHI}{$\varphi$}

\newcommand{\Pone}{P$\mathrm{_1}$}
\newcommand{\Ptwo}{P$\mathrm{_2}$}
\newcommand{\VG}{\ensuremath{V_g}\xspace}
\newcommand{\VD}{\ensuremath{V_d}\xspace}
\newcommand{\VBG}{$V\mathrm{_{bg}}$}
\newcommand{\IDS}{\ensuremath{I_{ds}}\xspace}
\mathnotation{\ION}{I_\text{on}}
\mathnotation{\IOFF}{I_\text{off}}
\newcommand{\GS}{\ensuremath{\Gamma_{\mathrm{S}}}\xspace}
\newcommand{\GD}{\ensuremath{\Gamma_{\mathrm{D}}}\xspace}
\newcommand{\GL}{\ensuremath{\Gamma_{\mathrm{L}}}\xspace}
\newcommand{\GR}{\ensuremath{\Gamma_{\mathrm{R}}}\xspace}
\newcommand{\GIN}{\ensuremath{\Gamma_{\mathrm{in}}}\xspace}
\newcommand{\GDEUX}{\ensuremath{\Gamma_{\mathrm{2}}'}\xspace}
\mathnotation{\CT}{\Delta}
\mathnotation{\AT}{\mathcal{T}}
\newcommand{\epsun}{\ensuremath{\epsilon_1}\xspace}
\newcommand{\epsdeux}{\ensuremath{\epsilon_2}\xspace}

\newcommand{\EConetwo}{$E_{C12}$}
\newcommand{\ZIMP}{z$_{\mathrm{imp}}$}

\mathnotation{\Do}{\mathrm{D}^0 \xspace}
\mathnotation{\Dion}{\mathrm{D}^+ \xspace}
\mathnotation{\Ddouble}{\mathrm{D}^- \xspace}

\mathnotation{\Restime}{R' \xspace}

\mathnotation{\GDR}{\Gamma_{2,R} \xspace}
\mathnotation{\GDL}{\Gamma_{2,L} \xspace}
\mathnotation{\GDS}{\Gamma_{2,S} \xspace}
\mathnotation{\GDD}{\Gamma_{2,D} \xspace}
\mathnotation{\TD}{T_{2,R} \xspace}
\mathnotation{\trie}{{\mathrm{e}^-}}
\mathnotation{\trih}{{\mathrm{h}^+}}

\mathnotation{\sigz}{\hat{\sigma}_z \xspace}
\mathnotation{\sigx}{\hat{\sigma}_x \xspace}
\mathnotation{\Bzero}{{\vec{B}}_0 \xspace}

\newcommand{\quantum}{\ensuremath{e^2/h}}

\usepackage[squaren,Gray]{SIunits}

\usepackage{blindtext}
\usepackage{enumitem}
\usepackage{xcolor}

\usepackage{aasmacros}
\usepackage{apacite}
\usepackage{natbib}
\setcitestyle{aysep={}} 
%\usepackage{breakcites}
%\usepackage{cite}

\def\d{{\mathrm d}}
%\newcommand{\degree}{\ensuremath{^\circ}}
%% --------------------------------------

\usepackage{silence}

\WarningFilter{minitoc(hints)}{W0023}
\WarningFilter{minitoc(hints)}{W0028}
\WarningFilter{minitoc(hints)}{W0030}
\WarningFilter{minitoc(hints)}{W0024}

\usepackage{longtable}
\setlength{\parskip}{0pt}
\usepackage{indentfirst}
\usepackage{subfig}

\AtBeginDocument{%
\hypersetup{
  %colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = Maroon, %Colour of internal links
  citecolor   = blue, %Colour of citations
}}

